J-PARSE: Jacobian-based Projection Algorithm for Resolving Singularities Effectively in Inverse Kinematic Control of Serial Manipulators

J-PARSE is an algorithm for smooth first-order inverse kinematic control of a serial manipulator near kinematic singularities. The commanded end-effector velocity is interpreted component-wise, according to the available mobility in each dimension of the task space. First, a substitute ''Safety'' Jacobian matrix is created, keeping the aspect ratio of the manipulability ellipsoid above a threshold value. The desired velocity is then projected onto non-singular and singular directions, and the latter projection scaled down by a factor informed by the altered mobility. A right-inverse of the non-singular Safety Jacobian is applied to the modified command. In the absence of joint limits and collisions, this ensures safe transition into and out of low-mobility configurations, guaranteeing locally stable reaching behavior towards target poses within, on the boundary of, and outside the workspace. The behavior is further guaranteed to be locally asymptotically stable if the starting and target configurations are not exactly singular, even if they are nearly singular. Velocity control with J-PARSE is benchmarked against approaches from the literature, illustrating its use of a single tuning parameter to simultaneously achieve high reaching accuracy and stable behavior. Applications in teleoperation, servoing, and learning are demonstrated. Videos and code are available at https://jparse-manip.github.io/.

==> glossary.tex <==
% Latex glossaries: https://www.overleaf.com/learn/latex/glossaries
%example: \acrshort{lfd} or \acrfull{lfd}; or \gls{lfd}. As we will not want to list the glossary, please use the asterisk: \gls*{--}; And if you use \gls{}, it will put the full acronym the first time it is called, then the shortened version there-after. \acrfull{} will force full form
\usepackage[acronym,nomain,nonumberlist]{glossaries}
\makeglossaries
%
%Example: \newacronym{name_you_call}{Short_form}{Full_form} %then just \gls{name_you_call}, and if you want to restate the full: \acrfull{name_you_call}
% To get plural \glspl{name_you_call}

\newacronym{ROS}{ROS}{Robot Operating System}
\newacronym{SVD}{SVD}{Singular Value Decomposition}
\newacronym{DLS}{DLS}{Damped Least Squares}
\newacronym{EDLS}{EDLS}{Exponential Damped Least Squares}
\newacronym{PID}{PID}{Proportional Integral Derivative}
\newacronym{DoF}{DoF}{degrees-of-freedom}
\newacronym{DDPM}{DDPMs}{Denoising Diffusion Probabilistic Models}
\newacronym{MSE}{MSE}{Mean Squared Error}
\newacronym{FiLM}{FiLM}{Feature-wise Linear Modulation}
\newacronym{J-PARSE}{J-PARSE}{Jacobian-based Projection Algorithm for Resolving Singularities Effectively}


